Planck 2015 results. III. LFI systematic uncertainties

We present the current accounting of systematic effect uncertainties for the Low Frequency Instrument (LFI) that are relevant to the 2015 release of the Planck cosmological results, showing the robustness and consistency of our data set, especially for polarization analysis. We use two complementary approaches: (i) simulations based on measured data and physical models of the known systematic effects; and (ii) analysis of difference maps containing the same sky signal ("null-maps"). The LFI temperature data are limited by instrumental noise. At large angular scales the systematic effects are below the cosmic microwave background (CMB) temperature power spectrum by several orders of magnitude. In polarization the systematic uncertainties are dominated by calibration uncertainties and compete with the CMB $E$-modes in the multipole range 10--20. Based on our model of all known systematic effects, we show that these effects introduce a slight bias of around $0.2\,\sigma$ on the reionization optical depth derived from the 70\,GHz $EE$ spectrum using the 30 and 353\,GHz channels as foreground templates. At 30\,GHz the systematic effects are smaller than the Galactic foreground at all scales in temperature and polarization, which allows us to consider this channel as a reliable template of synchrotron emission. We assess the residual uncertainties due to LFI effects on CMB maps and power spectra after component separation and show that these effects are smaller than the CMB amplitude at all scales. We also assess the impact on non-Gaussianity studies and find it to be negligible. Some residuals still appear in null maps from particular sky survey pairs, particularly at 30 GHz, suggesting possible straylight contamination due to an imperfect knowledge of the beam far sidelobes.

==> 04-211_polangle.tex <==
The reference frame in which each scanning beam (simulated with \texttt{GRASP} and reconstructed from Jupiter transits) was referred, is defined by the three angles $\theta_\textrm{uv}$, $\phi_\textrm{uv}$, and $\psi_\textrm{uv}$ reported in Table 5 of the \cite{planck2014-a03}. 
As described in \cite{planck2014-a05}, the selected frames imply that the power peak of the co-polar component lies along the main beam pointing direction, and a minimum in the cross-polar component appears in the same direction. 
In particular, the major axis of the polarization ellipse is along the x-axis for the radiometer side arm (S) and it is aligned with y- for the radiometer main arm (M). 
This means that, very close to the beam pointing direction, the main beam can be assumed to be linearly polarized; the x-axis of the main beam frame can be assumed to
be the main beam polarization direction for the radiometers S; and the y-axis of the main beam frame can be assumed to be the main beam polarization direction for the radiometers M.
The three angles $\theta_\textrm{uv}$, $\phi_\textrm{uv}$, and $\psi_\textrm{uv}$ were defined through optical simulations performed coupling the LFI feed horns to the Planck telescope, considering both the optical and radiometer bandshapes.
The $\psi_\textrm{pol}$ angle, reported in the same table, quantifies the alignement of the main beam polarization direction with respect to the x-axis of the main beam frame.
Therefore, the main beam pola\-ri\-zation angle ($\psi$) is defined by the sum of the two angles $\psi_\textrm{uv}$ and $\psi_\textrm{pol}$ (i.e., $\psi$ = $\psi_\textrm{uv}$ + $\psi_\textrm{pol}$), where $\psi_\textrm{pol}$ is supposed to be 0 or 90 degrees for the side and main arms, respectively.
In reality, in some cases $\psi_\textrm{pol}$ is slightly different to the ideal case because there is a tiny misalignment induced by the optical and radiometer behavior across the band.
In practice, the angle $\psi_\textrm{pol}$ varies of about $\pm$ 0.5$^\circ$ across the band and, taking also into account the radiometer bandshapes, we found the misalignment reported in the LFI RIMO, that are at most 0.5$^\circ$ far from the nominal values. 

A different approach could be to use the polarization angles derived from Crab observations.
The values derived from Crab observations are under investigation.
In the current release we have decided to use the values derived from \texttt{GRASP} simulations, since our optical model is well constrained by the main beam recostruction carried out with seven Jupiter transits, and to combine the simulated values with the measured uncertainties derived from the Crab observations.
  


==> 042_07_assessment_bandpass_mismatch.tex <==
\textit{Agenda:}

\textit{Compare leakage maps from }

\begin{itemize}
  \item \textit{different input data (effect of dodgy ancilliary data)}
  \item \textit{different physical models (e.g. power law vs GALPROP synchrotron spectra)}
  \item \textit{different CS algorithms (Commander vs Miramare)}
  \item \textit{different angular resolutions (hence SNR per pixel)}
  \item \textit{Assess impact of position angle uncertain on estimates of a-factors}
  \item \textit{Final combined error assessment \& reliability check}
\end{itemize}


==> figures/sidelobes_maura.tex <==
\subsubsection{Far sidelobes}
\label{sec_overview_far_sidelobes}
The far sidelobes are a source of systematic errors because they pick-up radiation far from the telescope line of sight and give rise to the so-called straylight contamination. The LFI 30\,GHz channel is particularly sensitive to the straylight contamination because the diffuse Galactic emission components are rather strong at this frequency, and the far sidelobe level of the 30\,GHz beams is significantly higher with respect to the other beams. The interested reader can find more details about the far sidelobes properties of the LFI beams in \citet{sandri2010}.
Straylight impacts the measurements in two ways: it directly contaminates the maps, and it affects the photometric calibration. In this latter case, the straylight could be a significant fraction of the measured signal that is compared with the calibrator itself (i.e., the Dipole), causing a systematic error in the recovered calibration constants. This error varies with time, depending on the orientation of the Galactic plane with respect to the line of sight.

In the 2013 release we did not correct the LFI data for the straylight contamination and we just estimated the residual uncertainty in the final maps and power spectra (see Table 2 and Fig.~1 of \citet{planck2013-p02a}). 
Accurate recovery of the CMB polarization, instead, required to consider properly this effect both in the calibration phase and in the production of the calibrated timelines. This is particularly true at 30\,GHz, while at 44 and 70\,GHz the straylight spurious signal is small compared to the CMB, both in temperature and polarization (see the green dotted spectra in Fig.~\ref{fig_systematic_effects_power_spectrum}).
We performed straylight correction in two steps: first, we calibrated the data accounting for the straylight contamination in the sky signal and then we removed it from the data themselves. To estimate the straylight signal we assume a fiducial model of the sidelobes based on \texttt{GRASP} beams and radiometer band shapes, as well as a fiducial model of the sky emission based on simulated temperature and polarization maps. We discuss the details of these procedures in Sect.~7.1 and 7.4 of \citet{planck2014-a03} and Sect.~2 of \citet{planck2014-a06}.

Accounting for the straylight signal in the analysis improves the data quality but arouses two questions: how well the beam model represents the real optical response and what are the residual uncertainties caused by a non perfect straylight removal. These questions could be addressed with Monte Carlo \texttt{GRASP} simulations of several beams that are then used in the analysis of simulated timelines generated starting from a fiducial sky and beam pattern. These simulations, however, require massive optical computations that were not affordable in the context of this data release. 

In this work we deal with this issue in two ways: on one side we do not add this effect in our simulations assuming a perfect straylight removal, on the other side we check for potential residual effects with null tests between adjoining surveys, which are particularly sensitive to straylight. We discuss these tests in Sect.~\ref{sec_assessment_null_tests} and summarize their results in Fig.~\ref{fig_ssodd-sseven-null}.

\subsubsection{Near sidelobes}
\label{sec_overview_near_sidelobes}

The \textit{near sidelobes} are defined as the region of the beam pattern in the angular range extending between the main beam angular limit\footnote{The main beam is defined as extending to 1.9, 1.3, and 0.9 degrees at 30, 44, and 70\,GHz, respectively. } and 5$^\circ$. Fig.~\ref{fig_intermediate_sidelobes} shows a typical beam pattern and highlights the near sidelobes region. We see that the power level of such lobes is up to 10 dBi (i.e., about --40 dB at 30\,GHz, --50 dB at 70\,GHz) and the shape of the near sidelobes is a typical diffraction pattern.
Near sidelobes can be a source of systematic effects when the main beam scans the sky near the Galactic plane or in the proximity of bright sources. In the parts of the sky dominated by diffuse emissions with little contrast in intensity, these lobes introduce a spurious signal of about $10^{-5}$ times the power entering the main beam. 
  We expect that the effect of near sidelobes on CMB measurements is small, provided that we properly mask the Galactic plane and the bright sources. For this reason we did not remove this effect from the data and assessed its impact generating simulated sky maps observed with and without the presence of near sidelobes in the beam and then taking the difference. We show and discuss such maps in Sect.~\ref{sec_assessment_simulations_optics_pointing} and the power spectrum of this effect in Fig.~\ref{fig_systematic_effects_power_spectrum}.

